Wayformer: Motion Forecasting via Simple & Efficient Attention Networks

Motion forecasting for autonomous driving is a challenging task because complex driving scenarios result in a heterogeneous mix of static and dynamic inputs. It is an open problem how best to represent and fuse information about road geometry, lane connectivity, time-varying traffic light state, and history of a dynamic set of agents and their interactions into an effective encoding. To model this diverse set of input features, many approaches proposed to design an equally complex system with a diverse set of modality specific modules. This results in systems that are difficult to scale, extend, or tune in rigorous ways to trade off quality and efficiency. In this paper, we present Wayformer, a family of attention based architectures for motion forecasting that are simple and homogeneous. Wayformer offers a compact model description consisting of an attention based scene encoder and a decoder. In the scene encoder we study the choice of early, late and hierarchical fusion of the input modalities. For each fusion type we explore strategies to tradeoff efficiency and quality via factorized attention or latent query attention. We show that early fusion, despite its simplicity of construction, is not only modality agnostic but also achieves state-of-the-art results on both Waymo Open MotionDataset (WOMD) and Argoverse leaderboards, demonstrating the effectiveness of our design philosophy

==> Wayformer Corl 2022/argoverse_tabular.tex <==
\begin{tabular}{ll|llll}
\toprule
\multicolumn{6}{c}{\textbf{Argoverse Leaderboard} ($k=6, d=2m, t=3s$)}                             \\ 
\multicolumn{2}{l|}{Models}                      & Brier-minFDE$^{*}$ ($\downarrow$) & minFDE ($\downarrow$) & MR ($\downarrow$)     & minADE ($\downarrow$)  \\ 
\midrule
\multicolumn{2}{l|}{LaneConv \cite{LaneConv}}                    & 2.0539       & 1.3622 & 0.1600 & 0.8703  \\
\multicolumn{2}{l|}{LaneRCNN \cite{LaneRCNN}}                    & 2.1470       & 1.4526 & 0.1232 & 0.9038  \\
\multicolumn{2}{l|}{mmTransformer \cite{StackedTransformer}}               & 2.0328       & 1.3383 & 0.1540 & 0.8346  \\
\multicolumn{2}{l|}{SceneTransformer \cite{SceneTA}}            & 1.8868       & 1.2321 & 0.1255 & 0.8026  \\
\multicolumn{2}{l|}{TNT \cite{zhao2020tnt}}                         & 2.1401       & 1.4457 & 0.1300 & 0.9400  \\
\multicolumn{2}{l|}{DenseTNT \cite{gu21dense_tnt}}                    & 1.9759       & 1.2858 & 0.1285 & 0.8817  \\
\multicolumn{2}{l|}{TPCN \cite{ye2021tpcn}}                        & 1.9286       & 1.2422 & 0.1333 & 0.8153  \\
\multicolumn{2}{l|}{MultiPath++ \cite{multipathpp}}                 & 1.7932       & 1.2144 & 0.1324 & 0.7897  \\
\multicolumn{2}{l|}{DCMS \cite{ye2022dcms}}                        & 1.7564       & \textbf{1.1350} & \textbf{0.1094} & \textbf{0.7659}  \\ 
\midrule
\midrule
\multirow{3}{*}{
\begin{tabular}{c}Wayformer\\ Early Fusion\end{tabular}
}  & \textbf{Attention}  &               &        &        &         \\ 
\cline{2-2}
                            & LQ + Multi-Axis &    \textbf{1.7408}          & 1.1615       &   0.1186     &  0.7675       \\
                            & LQ + Factorized & 1.7451       & 1.1625 & 0.1192 & 0.7672  \\
\bottomrule
\end{tabular}

==> Wayformer Corl 2022/relatedwork.tex <==
\section{Related Work}

\paragraph{Motion prediction architectures :}

Increasing interest in self-driving applications and the availability of benchmarks \cite{argoverse,lyft5,WOMD} has allowed motion prediction models to flourish.
Successful modeling techniques fuse multi-modal inputs that represent different static, dynamic, social and temporal aspects of the scene. 
% including the history of agent motion, the elements of the road graph (e.g.,
% lanes, stop lines, traffic light dynamic state) and agent interactions across time and space.
One class of models draws heavily from the computer vision literature, rendering inputs as a multichannel rasterized top-down image \cite{cui2019mtp,multipath,DBLP:journals/corr/LeeCVCTC17,DBLP:journals/corr/abs-1906-08945,casas2018intentnet,zhao2020tnt}.
In this approach, relationships between scene elements are rendered in the top down orthographic plane and modeled via spatio-temporal convolutional networks.
However, the localized structure of convolutions is well suited to processing image inputs, but is not effective at capturing the long range spatio-temporal relationships.
A popular alternative is to use an entity-centric approach, where agent state history is typically encoded via sequence modeling techniques like RNNs \cite{multiheadAF,wimp2020,social-lstm,rhinehart2019precog} or temporal convolutions \cite{liang2020laneGCN}.
Road elements are approximated with basic primitives (e.g. piece-wise linear segments) which encode pose and semantic information.
Modeling relationships between entities is often presented as an information aggregation process, and models employ pooling \cite{zhao2020tnt,gao2020vectornet,social-lstm,social-gan,multiheadAF,DBLP:journals/corr/LeeCVCTC17}, soft-attention \cite{multiheadAF,zhao2020tnt} or graph neural networks \cite{casas2020spagnn,liang2020laneGCN,wimp2020}.
Like our proposed method, several recent models use Transformers \cite{vaswani2017attention}, which are a popular state-of-the-art choice for sequence modeling in NLP \cite{devlin2018bert,DBLP:journals/corr/abs-2005-14165}, and have  shown promise in core computer vision tasks such as detection \cite{carion20detr,DBLP:journals/corr/abs-1904-09925,DBLP:journals/corr/abs-2101-11605}, tracking \cite{DBLP:journals/corr/abs-2008-07725} and classification \cite{DBLP:journals/corr/abs-1904-09925,DBLP:journals/corr/abs-1906-05909}.

\paragraph{Iterative cross-attention}
A recent approach to encode multi-modal data is to sequentially process one modality at a time \cite{StackedTransformer,perceiver,Autobots}.
\cite{StackedTransformer} ingests the scene in the order \{agent history, nearby agents, map\}; they argue that it is computationally expensive to perform self-attention over multiple modalities at once.
\cite{Autobots} pre-encodes the agent history and contextual agents through self-attention and cross-attends to the map with agent encodings as queries.
The order of self-attention and cross-attention relies heavily on the designer's intuition and has, to our knowledge, not been ablated before.

\paragraph{Factorized Attention}
Flattening high dimensional data leads to long sequences which make  self-attention computationally prohibitive.
\cite{axialattn} proposed limiting each attention operation to a single axes to alleviate the computational costs and applied this technique to autoregressive generative modeling for images.
Similarly, \cite{vivit} factorize the spatial and temporal dimensions of the video input when constructing their self-attention based classifier.
This axis based attention, which gets applied in interleaved fashion across layers, has been adopted in Transformer-based motion forecasting models \cite{Autobots} and graph neural network approaches \cite{SpatioTemporalGT}.
The order of applying attention over \{temporal, social/spatial\} dimensions has been studied with two different common patterns: (a) Temporal first \cite{social-lstm,social-gan,bigat} (b) Social/Spatial first \cite{stgat,trajectronpp}.
In Section \ref{sec:partial}, we study a `sequential' mode 
% where we apply repeatedly attention over the temporal dimension first, 
and contrast it with interleaved mode where interleave dimensions of attention similar to \cite{Autobots}. 

\paragraph{Multimodal Encoding}
\cite{agentformer} argued that attending to temporal and spatial dimensions independently leads to loss of information.
Moreover, allowing all inputs to self-attend to each other early on the encoding process reduces complexity and the need to handcraft architectures to address the scaling of computation for transformers with the increase in the input sequence length \cite{perceiver-io}.
However, self-attention is known to be computationally expensive for large inputs \cite{transformerbenchmark}, and recently there has been huge interest in approaches improving its scalability.
For a complete discussion of previous works, we refer the reader to the comprehensive survey \cite{efficientTransformers}.
One compelling approach is to use learned latent queries to decouples the number of query vectors of a Transformer encoder from the original input sequence length \cite{settransformer}.
This allows us to set the resolution of the Transformer output to arbitrary scales independent of the input, and flexibly tune model computational costs.
This approach is appealing since it does not assume any structure in the input and has proven effective in fusing multimodal inputs \cite{perceiver-io}. We take inspiration from such frameworks and present a study of their benefits when applied to the task of motion forecasting in the self-driving domain. 


==> Wayformer Corl 2022/result_table.tex <==
\begin{tabular}{ll|lllll|llll}
\toprule
\multicolumn{2}{l}{} & \multicolumn{5}{|c|}{\textbf{Waymo Open Motion Dataset}} & \multicolumn{4}{c}{\textbf{Argoverse Dataset}}  \\ 
\multicolumn{2}{l|}{Models} & minFDE ($\downarrow$) & minADE  ($\downarrow$) & MR  ($\downarrow$)  & Overlap ($\downarrow$) & mAP$^{*}$ ($\uparrow$) &
Brier-minFDE$^{*}$ ($\downarrow$) & minFDE ($\downarrow$) & MR ($\downarrow$)     & minADE ($\downarrow$)  \\ 
\midrule
%\multicolumn{2}{l|}{SimpleCNNOnRaster \cite{konev2021motioncnn}} & {1.494 & 0.740 & 0.209 & 0.156 & 0.214} & \multicolumn{4}{c}{} \\
\multicolumn{2}{l|}{SceneTransformer \cite{SceneTA}} & 1.212 & 0.612 & 0.156 & 0.147 & 0.279 & 1.8868       & 1.2321 & 0.1255 & 0.8026  \\
%\multicolumn{2}{l|}{HDGT \cite{hdgt}} & {1.206 & 0.593 &  0.151 & - & 0.285} & \multicolumn{4}{c}{} \\
%\multicolumn{2}{l|}{AIR \cite{air2}} & {0.829 & 0.502 & 0.185 & 0.033 & 0.315} & \multicolumn{4}{c}{} \\
\multicolumn{2}{l|}{DenseTNT \cite{gu21dense_tnt}} & 1.551 & 1.039 & 0.157 & 0.178   & 0.328 & 1.9759       & 1.2858 & 0.1285 & 0.8817 \\
%\multicolumn{2}{l|}{ReCoAt \cite{recoat}} & {0.773  & 0.403  & 0.166  & 0.032 & 0.348} & \multicolumn{4}{c}{}  \\
%\multicolumn{2}{l|}{Kraken-NMS (Yandex SDG)} & {1.395 & 0.673 & 0.185 & 0.142 & 0.365} & \multicolumn{4}{c}{} \\
\multicolumn{2}{l|}{MultiPath \cite{multipath}} & 2.040 & 0.880 & 0.345 & 0.166 & 0.409 & - & - & - & - \\
\multicolumn{2}{l|}{MultiPath++ \cite{multipathpp}} & 1.158  & 0.556  & 0.134  & 0.131 & 0.409 & 1.7932       & 1.2144 & 0.1324 & 0.7897  \\
\multicolumn{2}{l|}{LaneConv} & - & - & - & - & -  &                      2.0539       & 1.3622 & 0.1600 & 0.8703  \\
\multicolumn{2}{l|}{LaneRCNN \cite{LaneRCNN}} & - & - & - & - & - &                     2.1470       & 1.4526 & 0.1232 & 0.9038  \\
\multicolumn{2}{l|}{mmTransformer \cite{StackedTransformer}} & - & - & - & - & -               & 2.0328       & 1.3383 & 0.1540 & 0.8346 \\
\multicolumn{2}{l|}{TNT \cite{zhao2020tnt}}  & - & - & - & - & -                        & 2.1401       & 1.4457 & 0.1300 & 0.9400 \\
\multicolumn{2}{l|}{DCMS \cite{ye2022dcms}}      & - & - & - & - & -                   & 1.7564       & \textbf{1.1350} & \textbf{0.1094} & \textbf{0.7659}  \\ 
\midrule
\multicolumn{1}{l}{\multirow{3}{*}{\begin{tabular}{c}Wayformer\\ Early Fusion\end{tabular}}} & \textbf{Attention}  &  &  &  &  & & & & & \\ 
\cline{2-2}
 & LQ $+$ Multi-Axis & 1.128 & \textbf{0.545} & \textbf{0.123} & \textbf{0.127} & \textbf{0.419} & \textbf{1.7408}          & 1.1615       &   0.1186     &  0.7675 \\
& LQ $+$ Factorized & \textbf{1.126} & \textbf{0.545}  & \textbf{0.123} & \textbf{0.127} & 0.412 & 1.7451       & 1.1625 & 0.1192 & 0.7672 \\
\bottomrule
\end{tabular}



\begin{comment}
\midrule

\midrule


\midrule
\midrule

\end{comment}

==> Wayformer Corl 2022/womd_tabular.tex <==
\begin{tabular}{ll|lllll} 
\toprule
\multicolumn{7}{c}{\textbf{Waymo Open Motion Dataset}}  \\ 
\midrule
\multicolumn{2}{l|}{Models} & minFDE ($\downarrow$) & minADE  ($\downarrow$) & MR  ($\downarrow$)  & Overlap ($\downarrow$) & mAP$^{*}$ ($\uparrow$)  \\ 
\midrule
\multicolumn{2}{l|}{SimpleCNNOnRaster \cite{konev2021motioncnn}} & 
1.494 &
0.740 &
0.209 &
0.156 &
0.214 \\
\multicolumn{2}{l|}{SceneTransformer \cite{SceneTA}} & 1.212 & 0.612 & 0.156 & 0.147 & 0.279  \\
\multicolumn{2}{l|}{HDGT \cite{hdgt}} & 1.206 & 0.593 &  0.151 & - & 0.285 \\
\multicolumn{2}{l|}{AIR \cite{air2}} & 0.829 & 0.502 & 0.185 & 0.033 & 0.315 \\
\multicolumn{2}{l|}{DenseTNT \cite{gu21dense_tnt}} & 1.551 & 1.039 & 0.157 & 0.178   & 0.328 \\
\multicolumn{2}{l|}{ReCoAt \cite{recoat}} & 0.773  & 0.403  & 0.166  & 0.032 & 0.348  \\
\multicolumn{2}{l|}{Kraken-NMS (Yandex SDG)} & 1.395 & 0.673 & 0.185 & 0.142 & 0.365 \\
\multicolumn{2}{l|}{MultiPath \cite{multipath}} & 2.040 & 0.880 & 0.345 & 0.166 & 0.409 \\
\multicolumn{2}{l|}{MultiPath++ \cite{multipathpp}} & 1.158  & 0.556  & 0.134  & 0.131 & 0.409  \\

\midrule
\midrule
\multicolumn{1}{l}{\multirow{3}{*}{\begin{tabular}{c}Wayformer\\ Early Fusion\end{tabular}}} & \textbf{Attention}  &  & &  &  &  \\ 
\cline{2-2}
 & LQ $+$ Multi-Axis & 1.128 & \textbf{0.545} & \textbf{0.123} & \textbf{0.127} & \textbf{0.419} \\
& LQ $+$ Factorized & \textbf{1.126} & \textbf{0.545}  & \textbf{0.123} & \textbf{0.127} & 0.412  \\
\bottomrule
\end{tabular}
